Exploring Machine Teaching with Children

Iteratively building and testing machine learning models can help children develop creativity, flexibility, and comfort with machine learning and artificial intelligence. We explore how children use machine teaching interfaces with a team of 14 children (aged 7-13 years) and adult co-designers. Children trained image classifiers and tested each other's models for robustness. Our study illuminates how children reason about ML concepts, offering these insights for designing machine teaching experiences for children: (i) ML metrics (e.g. confidence scores) should be visible for experimentation; (ii) ML activities should enable children to exchange models for promoting reflection and pattern recognition; and (iii) the interface should allow quick data inspection (e.g. images vs. gestures).

==> arxiv2021 VLHCC KidsTeaMa(1)/reviews.tex <==
coordinator review
score 2/5

  Overall Rating

    Probably reject: I would argue for rejecting this paper.

  The Review

    (blank)

  The Meta Review

    All reviewers agree that this submission is clearly relevant to IDC, and that the
    contributions have merit as an early effort to teach machine learning concepts to
    young children. The reviewers also praise the clarity of some portions of the
    paper. However, all reviewers also raise significant concerns about the overall
    presentation, particularly with respect to the methodology, and missing details
    that suggest this submission is not quite publication-ready.

    R2 and R3 both question whether the methods described in the paper can really be
    described as co-design. The reviewers are not questioning the appropriateness of
    the methods used but rather the terminology.

    R2 and R3 found the paper lacking in depth in places and suggest that more
    discussion and synthesis of the design implications (R2) and overall conclusions
    (R2, R3) could help to strengthen the paper. Both reviewers point out some
    noteworthy and potentially significant findings in this work but more discussion
    is needed to bring them to light.

    R1 and R3 raise concerns about the selection criteria for participants.
    Importantly, R3 comments that there is not enough information about the selection
    and consent procedures to meet IDC community standards.

    R2 and R3 make several constructive suggestions to improve the clarity of the
    paper and highlight some additional related work that should be included.

    To summarize, the reviewers see a lot of potential in the work but question
    whether it is ready for publication at this time. I encourage the authors to
    consider incorporating all of the reviewers’ feedback. I also encourage the
    authors to consider submitting a revised version of this submission to the Late
    Breaking Work track (deadline April 12th).

----------------------------------------------------------------

reviewer 1 review
score 3/5

  Overall Rating

    Borderline: Overall I would not argue for accepting this paper.

  Expertise

    Knowledgeable

  The Review

    This paper presents an interesting dimension about machine teaching and how
    machine teaching applications can expose children to machine learning concepts.
    and the scope of the study is related to the IDC conference. The research problem
    and study’s objectives are clearly discussed in the introduction section.
    However, the sample size, selection criteria for choosing participants, and
    methodology used in this study make it difficult to generalize its result or draw
    any conclusions about the validity of the study, this study is one of the early
    efforts that tries to teach machine learning concepts to children 7-13 years old
    and can provide new insights into this domain.

----------------------------------------------------------------

reviewer 2 review
score 3/5

  Overall Rating

    Borderline: Overall I would not argue for accepting this paper.

  Expertise

    Knowledgeable

  The Review

    This work presents a study with children interacting with Teachable Machine in a
    way similar to existing work (Hitron et al. 2019) but with facilitation from adult
    designers ("co-design" an ML model with a well-performing image classifier). The
    activity is designed by specifying different features defined in the machine
    teaching space in prior work (Zhu et al. 2018). Under the high-level goal of
    designing teachable interfaces for children, the research question for this paper
    is "What are the key behaviors characterizing children’s interactions with a
    teachable interface such as the Google Teachable Machine?" The results reveal (1)
    how children interpreted confidence scores, (2) how children iterated their
    classifier by modifying the training dataset, (3) how children composed diverse
    examples, (4) how children conceptualized, and (5) tackled noise. Each part of the
    results from this study with children is compared with the results from the prior
    work about adult non-experts (Yang et al. 2018, Hong et al. 2020). Researchers
    extracted three design implications for teachable interfaces based on the
    empirical data, including (1) revealing confidence scores, (2) model swapping, (3)
    quick data inspection.

    • Significance of the paper's contribution to IDC and the benefit that others can
    gain from the contribution.
    The work is one of the early efforts investigating teachable machines for
    children. To study the design of teachable machine interfaces for children, this
    work started with observing and analyzing children's interaction with Google
    Teachable Machine. The paper provided rich study observations and generated design
    insights for teachable interface design for children. I am really looking forward
    to learning more about the teachable interface being developed by the research
    team based on these two study sessions. However, I am not sure if the contribution
    from this paper is significant and innovative enough to be a stand-only paper
    without proposing and evaluating their own design of teachable interfaces for
    children, especially considering Google Teachable Machine and similar platforms
    have been widely used/evaluated in many existing works introducing AI/ML to novice
    learners, and similar design guidelines have been proposed in previous work as
    well (but maybe in a more general context of AI for K-12).

    The "co-design" used in the paper is confusing since the actual co-design product
    from the study is not exactly aligned with the overall design goal of this
    research. Co-designing (i.e. building) an ML model with an adult co-designer by
    using GoogleTeaMa is similar to adults providing facilitation while children
    interacting with Google teachable machine in this work "Vartiainen, H., Tedre, M.,
    & Valtonen, T. (2020). Learning machine learning with very young children: Who is
    teaching whom?. International journal of child-computer interaction, 25, 100182."

    Though researchers compare the results from children with prior work on adult non-
    experts, it also makes me wonder about more in-depth and synthesized design
    implications or final conclusions on if teachable machine interfaces for children
    should differ from the teachable interfaces for adult non-experts. This could be a
    significant and innovative contribution but it is currently not explicitly
    synthesized and stated.

    • Validity of the work presented: how confidently can researchers and
    practitioners use the results?
    The work mainly adopted the thematic analysis for data analysis. However, there is
    no clear report of the coding scheme of thematic codes (for both a priori codes
    and emergent codes) and the coding results in the end.

    • Presentation clarity:
    The paper was overall well organized and presented clearly. For future
    improvements, I would like to mention a few places in the paper that are unclear
    to me.

    For study design, is there any difference between the two iterations of the
    session? It is unclear about the background of adult co-designers in the work: are
    they researchers? are they aware that the major study purpose? How did the session
    design make use of the technology immersion approach?

    There are no specific figures showing what teachable interfaces look like for this
    codesign study with children. Although the authors mentioned that they made use of
    an existing platform and the interaction process it's similar to prior work, I
    still would recommend making it clear and concrete in this paper itself.

    • Relevant previous work: is prior work adequately reviewed?
    I would suggest a few existing papers that may offer some insights but not
    currently included in the reference, such as:
    Vartiainen, H., Tedre, M., & Valtonen, T. (2020). Learning machine learning with
    very young children: Who is teaching whom?. International journal of child-
    computer interaction, 25, 100182.

    Stefania Druga, Sarah T Vu, Eesh Likhith, and Tammy Qiu. 2019. Inclusive AI
    literacy for kids around the world. In Proceedings of FabLearn 2019. 104–111.

    Long, D., & Magerko, B. (2020, April). What is AI literacy? Competencies and
    design considerations. In Proceedings of the 2020 CHI Conference on Human Factors
    in Computing Systems (pp. 1-16).

    Toivonen, T., Jormanainen, I., Kahila, J., Tedre, M., Valtonen, T., & Vartiainen,
    H. (2020, July). Co-Designing Machine Learning Apps in K–12 With Primary School
    Children. In 2020 IEEE 20th International Conference on Advanced Learning
    Technologies (ICALT) (pp. 308-310). IEEE.

----------------------------------------------------------------

reviewer 3 review
score 3/5

  Overall Rating

    Borderline: Overall I would not argue for accepting this paper.

  Expertise

    Knowledgeable

  The Review

    The paper contributes a number of interesting insights into how children can be
    exposed to basic machine learning and artificial intelligence concepts without
    programming. These are related both to (1) the design of the interface/activity -
    i.e., revealing the confidence scores derived by a model and designing the
    interface to enable in-the-moment data inspection; and (2) the design of the
    learning activity - i.e., by designing activities that afford model swapping
    between children.

    The domain is timely and relevant, as teaching ML and AI is quickly becoming of
    increasing empirical interest in the IDC and broader computing education
    communities. The related work section seems comprehensive and positions the
    empirical purpose of the paper well.

    Methods
    I have some concerns with the presentation of the methodology. Specifically, there
    is little specification of selection and consent procedures with the children,
    which is key in the IDC community, in terms of: how were these particular
    participants selected? How was informed consent obtained?

    The paper would also have benefitted from an overview of the children’s
    backgrounds and to what extent they knew about machine learning already. The
    authors state that the children “were members of an intergenerational team
    practicing Cooperative Inquiry”. The language here is a bit unclear - to me it
    implies that the children were part of a group that regularly met for other
    Cooperative Inquiry tasks as well - but this needs clarification. ]

    Finally, in my perspective, the method adopted here stretches the traditional
    definition of Cooperative Inquiry a bit - the children were seemingly not involved
    in the design, other than testing a pedagogical design that was prepared by the
    authors. They were not asked to feed back on the design itself, other than talking
    about what they experienced during the learning process. This is completely fine,
    but I am not sure whether Cooperative Inquiry is the most appropriate terminology
    to use for the study design. The authors cite that their method is a form of
    technology immersion, however, technology immersion usually involves giving
    children a long period of time and freedom of choice about how they interact with
    the available technologies, rather than a set task [1].

    Discussion and contribution
    The Discussion feels a lacking given the rich insights in the results section -
    for example, I hoped for more nuance in the implication about how confidence
    scores should be presented. Is it always good for children to try to build 100%
    confident models? How might a system be designed to more critically engage them
    with what a “good” or “sufficient” confidence score is given a particular dataset?

    While model swapping is discussed, I also hoped for more on the other forms of
    pedagogical strategies that are important. For instance, the implications of the
    origami task set out (e.g., in terms of the types of noise it allowed the children
    to experience) as well as the level of adult/teacher support seemed to feature
    prominently in the Results. I hoped to see these returned to in the Discussion.

    I feel a deeper discussion would help highlight the contribution of the paper
    more.

    For these reasons, I am giving this paper a neutral score, as I feel that while
    there is a lot of good in this paper, there are some key areas that would be
    important to improve prior to publication.

    Finally, a couple of minor points:
    - There are a couple of references that seem to be repeated twice, specifically
    the two Touretzky ones from 2019.

    - The paper could do with a bit of an edit for clarity. E.g., see above comment
    about clarity of whether the children were involved in a longer term Cooperative
    Inquiry team. There are other instances of slightly unclear writing in the paper,
    e.g., p7 the sentence starting with "After the session ended" seems to be
    referring to both sessions, p7 "...participated in the design sessions over two
    years" is a bit ambiguous in that it sounds like the children were part of the
    team for two years, rather than just at one session each.

    - It is mentioned that many of the children were second generation immigrants -
    however, noting that IDC is an international conference, if this information is to
    be included, it feels important to say where the children were immigrants to - I
    assume USA, but this should be made explicit. More generally though I wonder why
    it's important to say that many of the children were second-generation (and to
    describe each child's ethnicity)? Is this aimed at being a marker of how inclusive
    the study was? If so, I would again make that explicit, and encourage the authors
    to say why they feel this is important information to include. While I understand
    that it may be relevant to the interpretation and generalizability of the
    findings, it feels strange to describe participants' ethnicities and other
    protected characteristics without adding further context/rationale about why they
    are important to note.

    [1] Druin, A., Bederson, B., Boltman, A., Miura, A., Knotts-Callahan, D., & Platt,
    M. (1998). Children as our technology design partners+.

==> reviews.tex <==
coordinator review
score 2/5

  Overall Rating

    Probably reject: I would argue for rejecting this paper.

  The Review

    (blank)

  The Meta Review

    All reviewers agree that this submission is clearly relevant to IDC, and that the
    contributions have merit as an early effort to teach machine learning concepts to
    young children. The reviewers also praise the clarity of some portions of the
    paper. However, all reviewers also raise significant concerns about the overall
    presentation, particularly with respect to the methodology, and missing details
    that suggest this submission is not quite publication-ready.

    R2 and R3 both question whether the methods described in the paper can really be
    described as co-design. The reviewers are not questioning the appropriateness of
    the methods used but rather the terminology.

    R2 and R3 found the paper lacking in depth in places and suggest that more
    discussion and synthesis of the design implications (R2) and overall conclusions
    (R2, R3) could help to strengthen the paper. Both reviewers point out some
    noteworthy and potentially significant findings in this work but more discussion
    is needed to bring them to light.

    R1 and R3 raise concerns about the selection criteria for participants.
    Importantly, R3 comments that there is not enough information about the selection
    and consent procedures to meet IDC community standards.

    R2 and R3 make several constructive suggestions to improve the clarity of the
    paper and highlight some additional related work that should be included.

    To summarize, the reviewers see a lot of potential in the work but question
    whether it is ready for publication at this time. I encourage the authors to
    consider incorporating all of the reviewers’ feedback. I also encourage the
    authors to consider submitting a revised version of this submission to the Late
    Breaking Work track (deadline April 12th).

----------------------------------------------------------------

reviewer 1 review
score 3/5

  Overall Rating

    Borderline: Overall I would not argue for accepting this paper.

  Expertise

    Knowledgeable

  The Review

    This paper presents an interesting dimension about machine teaching and how
    machine teaching applications can expose children to machine learning concepts.
    and the scope of the study is related to the IDC conference. The research problem
    and study’s objectives are clearly discussed in the introduction section.
    However, the sample size, selection criteria for choosing participants, and
    methodology used in this study make it difficult to generalize its result or draw
    any conclusions about the validity of the study, this study is one of the early
    efforts that tries to teach machine learning concepts to children 7-13 years old
    and can provide new insights into this domain.

----------------------------------------------------------------

reviewer 2 review
score 3/5

  Overall Rating

    Borderline: Overall I would not argue for accepting this paper.

  Expertise

    Knowledgeable

  The Review

    This work presents a study with children interacting with Teachable Machine in a
    way similar to existing work (Hitron et al. 2019) but with facilitation from adult
    designers ("co-design" an ML model with a well-performing image classifier). The
    activity is designed by specifying different features defined in the machine
    teaching space in prior work (Zhu et al. 2018). Under the high-level goal of
    designing teachable interfaces for children, the research question for this paper
    is "What are the key behaviors characterizing children’s interactions with a
    teachable interface such as the Google Teachable Machine?" The results reveal (1)
    how children interpreted confidence scores, (2) how children iterated their
    classifier by modifying the training dataset, (3) how children composed diverse
    examples, (4) how children conceptualized, and (5) tackled noise. Each part of the
    results from this study with children is compared with the results from the prior
    work about adult non-experts (Yang et al. 2018, Hong et al. 2020). Researchers
    extracted three design implications for teachable interfaces based on the
    empirical data, including (1) revealing confidence scores, (2) model swapping, (3)
    quick data inspection.

    • Significance of the paper's contribution to IDC and the benefit that others can
    gain from the contribution.
    The work is one of the early efforts investigating teachable machines for
    children. To study the design of teachable machine interfaces for children, this
    work started with observing and analyzing children's interaction with Google
    Teachable Machine. The paper provided rich study observations and generated design
    insights for teachable interface design for children. I am really looking forward
    to learning more about the teachable interface being developed by the research
    team based on these two study sessions. However, I am not sure if the contribution
    from this paper is significant and innovative enough to be a stand-only paper
    without proposing and evaluating their own design of teachable interfaces for
    children, especially considering Google Teachable Machine and similar platforms
    have been widely used/evaluated in many existing works introducing AI/ML to novice
    learners, and similar design guidelines have been proposed in previous work as
    well (but maybe in a more general context of AI for K-12).

    The "co-design" used in the paper is confusing since the actual co-design product
    from the study is not exactly aligned with the overall design goal of this
    research. Co-designing (i.e. building) an ML model with an adult co-designer by
    using GoogleTeaMa is similar to adults providing facilitation while children
    interacting with Google teachable machine in this work "Vartiainen, H., Tedre, M.,
    & Valtonen, T. (2020). Learning machine learning with very young children: Who is
    teaching whom?. International journal of child-computer interaction, 25, 100182."

    Though researchers compare the results from children with prior work on adult non-
    experts, it also makes me wonder about more in-depth and synthesized design
    implications or final conclusions on if teachable machine interfaces for children
    should differ from the teachable interfaces for adult non-experts. This could be a
    significant and innovative contribution but it is currently not explicitly
    synthesized and stated.

    • Validity of the work presented: how confidently can researchers and
    practitioners use the results?
    The work mainly adopted the thematic analysis for data analysis. However, there is
    no clear report of the coding scheme of thematic codes (for both a priori codes
    and emergent codes) and the coding results in the end.

    • Presentation clarity:
    The paper was overall well organized and presented clearly. For future
    improvements, I would like to mention a few places in the paper that are unclear
    to me.

    For study design, is there any difference between the two iterations of the
    session? It is unclear about the background of adult co-designers in the work: are
    they researchers? are they aware that the major study purpose? How did the session
    design make use of the technology immersion approach?

    There are no specific figures showing what teachable interfaces look like for this
    codesign study with children. Although the authors mentioned that they made use of
    an existing platform and the interaction process it's similar to prior work, I
    still would recommend making it clear and concrete in this paper itself.

    • Relevant previous work: is prior work adequately reviewed?
    I would suggest a few existing papers that may offer some insights but not
    currently included in the reference, such as:
    Vartiainen, H., Tedre, M., & Valtonen, T. (2020). Learning machine learning with
    very young children: Who is teaching whom?. International journal of child-
    computer interaction, 25, 100182.

    Stefania Druga, Sarah T Vu, Eesh Likhith, and Tammy Qiu. 2019. Inclusive AI
    literacy for kids around the world. In Proceedings of FabLearn 2019. 104–111.

    Long, D., & Magerko, B. (2020, April). What is AI literacy? Competencies and
    design considerations. In Proceedings of the 2020 CHI Conference on Human Factors
    in Computing Systems (pp. 1-16).

    Toivonen, T., Jormanainen, I., Kahila, J., Tedre, M., Valtonen, T., & Vartiainen,
    H. (2020, July). Co-Designing Machine Learning Apps in K–12 With Primary School
    Children. In 2020 IEEE 20th International Conference on Advanced Learning
    Technologies (ICALT) (pp. 308-310). IEEE.

----------------------------------------------------------------

reviewer 3 review
score 3/5

  Overall Rating

    Borderline: Overall I would not argue for accepting this paper.

  Expertise

    Knowledgeable

  The Review

    The paper contributes a number of interesting insights into how children can be
    exposed to basic machine learning and artificial intelligence concepts without
    programming. These are related both to (1) the design of the interface/activity -
    i.e., revealing the confidence scores derived by a model and designing the
    interface to enable in-the-moment data inspection; and (2) the design of the
    learning activity - i.e., by designing activities that afford model swapping
    between children.

    The domain is timely and relevant, as teaching ML and AI is quickly becoming of
    increasing empirical interest in the IDC and broader computing education
    communities. The related work section seems comprehensive and positions the
    empirical purpose of the paper well.

    Methods
    I have some concerns with the presentation of the methodology. Specifically, there
    is little specification of selection and consent procedures with the children,
    which is key in the IDC community, in terms of: how were these particular
    participants selected? How was informed consent obtained?

    The paper would also have benefitted from an overview of the children’s
    backgrounds and to what extent they knew about machine learning already. The
    authors state that the children “were members of an intergenerational team
    practicing Cooperative Inquiry”. The language here is a bit unclear - to me it
    implies that the children were part of a group that regularly met for other
    Cooperative Inquiry tasks as well - but this needs clarification. ]

    Finally, in my perspective, the method adopted here stretches the traditional
    definition of Cooperative Inquiry a bit - the children were seemingly not involved
    in the design, other than testing a pedagogical design that was prepared by the
    authors. They were not asked to feed back on the design itself, other than talking
    about what they experienced during the learning process. This is completely fine,
    but I am not sure whether Cooperative Inquiry is the most appropriate terminology
    to use for the study design. The authors cite that their method is a form of
    technology immersion, however, technology immersion usually involves giving
    children a long period of time and freedom of choice about how they interact with
    the available technologies, rather than a set task [1].

    Discussion and contribution
    The Discussion feels a lacking given the rich insights in the results section -
    for example, I hoped for more nuance in the implication about how confidence
    scores should be presented. Is it always good for children to try to build 100%
    confident models? How might a system be designed to more critically engage them
    with what a “good” or “sufficient” confidence score is given a particular dataset?

    While model swapping is discussed, I also hoped for more on the other forms of
    pedagogical strategies that are important. For instance, the implications of the
    origami task set out (e.g., in terms of the types of noise it allowed the children
    to experience) as well as the level of adult/teacher support seemed to feature
    prominently in the Results. I hoped to see these returned to in the Discussion.

    I feel a deeper discussion would help highlight the contribution of the paper
    more.

    For these reasons, I am giving this paper a neutral score, as I feel that while
    there is a lot of good in this paper, there are some key areas that would be
    important to improve prior to publication.

    Finally, a couple of minor points:
    - There are a couple of references that seem to be repeated twice, specifically
    the two Touretzky ones from 2019.

    - The paper could do with a bit of an edit for clarity. E.g., see above comment
    about clarity of whether the children were involved in a longer term Cooperative
    Inquiry team. There are other instances of slightly unclear writing in the paper,
    e.g., p7 the sentence starting with "After the session ended" seems to be
    referring to both sessions, p7 "...participated in the design sessions over two
    years" is a bit ambiguous in that it sounds like the children were part of the
    team for two years, rather than just at one session each.

    - It is mentioned that many of the children were second generation immigrants -
    however, noting that IDC is an international conference, if this information is to
    be included, it feels important to say where the children were immigrants to - I
    assume USA, but this should be made explicit. More generally though I wonder why
    it's important to say that many of the children were second-generation (and to
    describe each child's ethnicity)? Is this aimed at being a marker of how inclusive
    the study was? If so, I would again make that explicit, and encourage the authors
    to say why they feel this is important information to include. While I understand
    that it may be relevant to the interpretation and generalizability of the
    findings, it feels strange to describe participants' ethnicities and other
    protected characteristics without adding further context/rationale about why they
    are important to note.

    [1] Druin, A., Bederson, B., Boltman, A., Miura, A., Knotts-Callahan, D., & Platt,
    M. (1998). Children as our technology design partners+.
